Multiple Quasiparticle Bound States in a Trap Created by a Local Superconducting Gap Variation

At low temperature, the concentration of quasiparticles observed in superconducting circuits far exceeds the predictions of microscopic BCS theory at equilibrium. As a source of dissipation, these excess quasiparticles degrade the performance of various devices. Therefore, understanding their dynamics, especially their recombination into Cooper pairs, is an active topic of current research. In disordered superconductors, spatial fluctuations in the superconducting gap can trap quasiparticles and modify their eigenspectrum. Since this spectrum plays a key role in quasiparticle dynamics, it must be carefully investigated. To this end, we introduce a toy model of a single trap. Specifically, we consider a shallow disk-shaped gap variation in a clean superconductor. Using a semiclassical approximation, we demonstrate the existence of multiple bound states and give the dependence of their number on the size and depth of the gap suppression. Extending our analysis beyond the semiclassical regime, in dimensions larger than one, we observe an infinite number of bound states very close to the gap edge, even for an arbitrarily small trap. These results deepen our understanding of trapped quasiparticles and may have important implications for their recombination in disordered superconductors.

==> Taylor_DVLP.tex <==

\section{Taylor dvlp}
\subsection{1D case}
We start from following 1D equation for quasiparticle energy:
\begin{equation}-2\arccos(1-2\tilde\epsilon)+4s\gamma\sqrt{1-\tilde\epsilon}=2n\pi, \qquad n\in\mathbb{N}\end{equation}


When considering $\tilde\epsilon \to 0$ we get: 

\begin{equation}-4\sqrt{\tilde\epsilon}+4s\gamma\Big(1-\frac{\tilde\epsilon}{2} \Big)=2n\pi\end{equation}

So for the ground state at $n=0$, when considering $s\gamma <<1$ such as we can neglect $s\gamma \tilde\epsilon$ and we recover \begin{equation}\tilde\epsilon_0\approx s^2\gamma^2\end{equation}


When $n>0$ and we consider $s\gamma >>1$, we can't neglect $s\gamma \tilde\epsilon$ and we get: 

\begin{equation}
\begin{split}
    &\sqrt{\tilde\epsilon} = s\gamma \Big( 1- \frac{\tilde \epsilon}{2}\Big) - \frac{n\pi}{2}
    \\
    &\tilde \epsilon = \Bigg[s\gamma\Big( 1- \frac{\tilde \epsilon}{2}\Big) - \frac{n\pi}{2}\Bigg]^2
    \\
    & \tilde \epsilon = s^2\gamma^2 (1 - \frac{\tilde \epsilon}{2})^2 + \frac{n^2\pi^2}{4} - s\gamma n\pi(1-\frac{\tilde\epsilon}{2})
    \\
    &\tilde \epsilon \approx s^2\gamma^2 -s\gamma n\pi + \frac{n^2\pi^2}{4} - \tilde\epsilon\Big(s^2\gamma^2-s\gamma n\pi\Big) 
    \\
    & \tilde \epsilon\big(1+ s^2\gamma^2-s\gamma n\pi\big)  \approx s^2\gamma^2 -s\gamma n\pi + \frac{n^2\pi^2}{4}
\end{split}
\end{equation}


As we are looking at $s\gamma >>1$ we get:
\begin{equation}
\begin{split}
    &\tilde \epsilon\approx 1+ \frac{1}{\big( s^2\gamma^2-s\gamma n\pi\big)}\frac{n^2\pi^2}{4}
    \approx 1+ \frac{n^2\pi^2}{4s^2\gamma^2}
\end{split}
\end{equation}

\textcolor{blue}{Sign pb I should obtain $1- \frac{n^2\pi^2}{4s^2\gamma^2}$}

\subsection{2D case:}

We now are looking at the following energy equation in the 2D case: 
\begin{equation}
    -2\arccos(1-2\tilde\epsilon)+4\gamma\sqrt{s^2-\ell^2}\sqrt{1-\tilde\epsilon}=2n\pi
\end{equation}

When considering $\tilde\epsilon\to0$ we get: 
\begin{equation}
    -4\sqrt{\tilde\epsilon}+4\gamma\sqrt{s^2-\ell^2}\big(1-\tilde\epsilon/2\big)=2n\pi
\end{equation}

If considering $n=\ell=0$ we get the same equation as for the 1D case and thus the result is the same. If we look at the other states for $n>0$ we get: 

\begin{equation}
\begin{split}
    &-\sqrt{\tilde\epsilon}+\gamma\sqrt{s^2-\ell^2}\big(1-\tilde\epsilon/2\big)=\frac{n\pi}{2}
    \\
    & \tilde\epsilon= \Bigg[ \gamma\sqrt{s^2-\ell^2}\big(1-\tilde\epsilon/2\big)-\frac{n\pi}{2} \Bigg ]^2
    \\
    & \tilde\epsilon= \Bigg[ \gamma^2(s^2-\ell^2)\big(1-\tilde\epsilon\big)+\frac{n^2\pi^2}{4} - {n\pi}\gamma\sqrt{s^2-\ell^2}\big(1-\tilde\epsilon/2\big)
\end{split}
\end{equation}

==> coefcc.tex <==

\
\\
From the two first equation we get:  
\begin{equation}
    A_1= \frac{G_1(k_{he}+q_{eh})(u_s v_0 - u_0 v_s) - F_1(k_{eh}-q_{eh})(u_0 u_s - v_0 v_s)}{2 q_{eh}(u_s^2-v_s^2)}
\end{equation}
\begin{equation}
    A_2= \frac{-G_1(k_{he}-q_{eh})(u_s v_0 - u_0 v_s) + F_1(k_{eh}+q_{eh})(u_0 u_s - v_0 v_s)}{2 q_{eh}(u_s^2-v_s^2)}
\end{equation}
\begin{equation}
    B_1= \frac{-F_1(k_{eh}-q_{he})(u_s v_0 - u_0 v_s) + G_1(k_{he}+q_{he})(u_0 u_s - v_0 v_s)}{2 q_{eh}(u_s^2-v_s^2)}
\end{equation}
\begin{equation}
    B_2= \frac{F_1(k_{eh}+q_{he})(u_s v_0 - u_0 v_s) - G_1(k_{he}-q_{he})(u_0 u_s - v_0 v_s)}{2 q_{eh}(u_s^2-v_s^2)}
\end{equation}


From the two other equations we get: 
\begin{widetext}
\begin{equation}
    A_1= \frac{-G_3 e^{-i2R(k_{he}+q_{eh})}(k_{he}-q_{eh})(u_s v_0 - u_0 v_s) - F_3e^{i2R(k_{eh}-q_{eh})}(k_{eh}+q_{eh})(u_0 u_s - v_0 v_s)}{2 q_{eh}(u_s^2-v_s^2)}
\end{equation}

 \begin{equation}
    A_2= \frac{G_3 e^{-i2R(k_{he}-q_{eh})}(k_{he}+q_{eh})(u_s v_0 - u_0 v_s) + F_3e^{i2R(k_{eh}+q_{eh})}(-k_{eh}+q_{eh})(u_0 u_s - v_0 v_s)}{2 q_{eh}(u_s^2-v_s^2)}
\end{equation}   

 \begin{equation}
    B_1= \frac{F_3e^{i2R(k_{eh}-q_{he})}(k_{eh}+q_{he})(u_s v_0 - u_0 v_s) - G_3e^{-i2R(k_{he}-q_{he})}(k_{he}-q_{he})(u_0 u_s - v_0 v_s)}{2 q_{eh}(u_s^2-v_s^2)}
\end{equation}   

 \begin{equation}
    B_2= \frac{F_3e^{i2R(k_{eh}+q_{he})}(k_{eh}-q_{he})(u_s v_0 - u_0 v_s) + G_3 e^{i2R(k_{he}+q_{he})}(k_{he}+q_{he})(u_0 u_s - v_0 v_s)}{2 q_{eh}(u_s^2-v_s^2)}
\end{equation}   
\end{widetext}

Let's determine now $F_1$ coefficient by taking $(k_{he}+q_{he}) B_1 + (k_{eh}-q_{he}) B_2 $ and $G_1$ by taking  $(k_{he}-q_{he}) B_1 + (k_{he}+q_{he}) B_2 $ such as we get the following equation: 
\begin{widetext}
\begin{align*}
\begin{split}
  %  F_1  = \frac{G_3 e^{-i 2Rk_{he}}\bigg[e^{i2Rq_{eh}}(k_{he}+q_{eh})^2 - e^{-i2Rq_{eh}}(k_{he}-q_{eh})^2\bigg](u_s v_0 - u_0 v_s) + F_3e^{-i 2Rk_{he}} \bigg[e^{-i 2Rq_{eh}} - e^{i 2R q_{eh}} \bigg](k_{he}-q_{eh})(k_{eh}+q_{eh})(u_0 u_s - v_0 v_s)}{\bigg[(k_{eh}+ q_{eh})(k_{he}+q_{eh}) - (k_{eh}- q_{eh})(k_{he}-q_{eh})(u_0 u_s - v_0 v_s) \bigg]}
   F_1  =& \frac{G_3 e^{-i 2Rk_{he}}\bigg[e^{i2Rq_{eh}}(k_{he}+q_{eh})^2 - e^{-i2Rq_{eh}}(k_{he}-q_{eh})^2\bigg](u_s v_0 - u_0 v_s)}{\bigg[ 2 q_{eh}(k_{eh}-k_{he})(u_0 u_s - v_0 v_s) \bigg]}
   \\
   & - \frac{F_3e^{-i 2Rk_{he}} \bigg[e^{-i 2Rq_{eh}} + e^{i 2R q_{eh}} \bigg](k_{he}-q_{eh})(k_{eh}+q_{eh})(u_0 u_s - v_0 v_s)}{\bigg[ 2 q_{eh}(k_{eh}-k_{he})(u_0 u_s - v_0 v_s) \bigg]}
\end{split}
\end{align*}
\begin{align*}
\begin{split}
  %  F_1  = \frac{G_3 e^{-i 2Rk_{he}}\bigg[e^{i2Rq_{eh}}(k_{he}+q_{eh})^2 - e^{-i2Rq_{eh}}(k_{he}-q_{eh})^2\bigg](u_s v_0 - u_0 v_s) + F_3e^{-i 2Rk_{he}} \bigg[e^{-i 2Rq_{eh}} - e^{i 2R q_{eh}} \bigg](k_{he}-q_{eh})(k_{eh}+q_{eh})(u_0 u_s - v_0 v_s)}{\bigg[(k_{eh}+ q_{eh})(k_{he}+q_{eh}) - (k_{eh}- q_{eh})(k_{he}-q_{eh})(u_0 u_s - v_0 v_s) \bigg]}
   G_1  =& \frac{G_3 e^{-i 2Rk_{he}}\bigg[e^{i2Rq_{eh}}(k_{he}+q_{eh})(k_{he}+ q_{eh}) - e^{-i2Rq_{eh}}(k_{he}-q_{eh})(k_{he}-q_{eh})\bigg](u_s v_0 - u_0 v_s)}{\bigg[ 2 q_{eh}(k_{eh}-k_{he})(u_0 u_s - v_0 v_s) \bigg]}
   \\
   & - \frac{F_3e^{-i 2Rk_{he}} \bigg[e^{-i 2Rq_{eh}}(k_{eh}+q_{eh})^2 + e^{i 2R q_{eh}(k_{eh}-q_{eh})^2} \bigg](u_0 u_s - v_0 v_s)}{\bigg[ 2 q_{eh}(k_{eh}-k_{he})(u_0 u_s - v_0 v_s) \bigg]}
\end{split}
\end{align*}
\end{widetext}



Let's also determine $F_1$ and $G_1$ by solving $(k_{eh}-q_{eh}) A_1 + (k_{eh}+q_{eh}) A_2 $




